Boundary layer formation in the quasigeostrophic model near nonperiodic rough coasts

We study the so-called homogeneous model of wind-driven ocean circulation, also known as the single-layer quasigeostrophic model. Our attention focuses on performing a complete asymptotic analysis that highlights boundary layer formation along the coastal line. We assume rough coasts without any particular structure, resulting in the study of a nonlinear PDE system for the western boundary layer in an infinite domain. As a consequence, we look for the solution in nonlocalized Sobolev spaces. Under this hypothesis, the eastern boundary layer exhibits a singular behavior at low frequencies far from the rough boundary leading to issues with convergence. The problem is tackled by imposing ergodicity properties. We establish the well-posedness of the governing boundary layer equations and the approximate solution. Our results generalize the ones in the paper of Bresch and G\'erard-Varet (Commun. Math. Phys. (1) 253: (2005), 81-119) in the context of periodic irregularities.

==> eastern/link_interior.tex <==
\subsection{Relation}\label{link}

We first establish a representation formula for $v$ in terms of the double-layer Stokes
potential.
\begin{lemma}\label{Bass_lemma11_equiv}
	Almost surely, $\Psi^1_e$ satisfies, for $X > 1$,
	\begin{eqnarray}\label{Bass_411}
	\Psi^1_{e}(\omega,y)&=&\int\limits_\mathbb{R}K(X, Y-Y)\Psi^1_{e}(\omega,Y',0)dY'\\
	&=&-\int\limits_\mathbb{R} Y'\partial_Y' G(X)\frac{1}{Y'}\int\limits_{0}^{Y'}\Psi^1_{e}(\omega,Y-s,0)ds\thinspace dY',\nonumber
	\end{eqnarray}
	where $K(X,Y)=\mathcal{F}$.
\end{lemma}

From Lemma \ref{lemma7_equiv}, we know that for $Y'\rightarrow K(X, Y-Y')$ is  $L^1(\mathbb{R})$, $|X|\geq 1$. Then, the equation of $\psi^1$ can be rewritten as follows
\begin{equation*}
\psi^1(X,Y)=\overline{\psi}_0+\sum_{q\in\mathbb{Z}}\int_{\mathbb{R}}K(X,Y')\left(\psi_0(Y-Y')-\overline{\psi}_0\right)\varphi_q(Y')dY'.
\end{equation*}

Let $m(X)=\int_{\mathbb{R}}K(X,Y)dY$, where $K=\mathcal{F}^{-1}\left(\xi\mapsto\chi(\xi)e^{-\lambda_1(\xi)X}\right)$. We have \begin{equation*}
\int_\mathbb{R}K(X,Y)dY= \widehat{K}(X,0)=\chi(0)e^{-\lambda_1(0)X}=1,\end{equation*} and, consequently, $m(X)=1$, when $X>0$.
Taking into account that $m(X)=1$, for all $X>0$, and integrating by parts yield
\begin{equation*}
\psi^1(X,Y)=\overline{\psi}_0-\sum_{q\in\mathbb{Z}}\int_{\mathbb{R}}\partial_{Y'}K(X,Y')\int_0^{Y'}\left(\psi_0(Y-Y_1)-\overline{\psi}_0\right)dY_1\varphi_q(Y')dY'.
\end{equation*}
Moreover, 
\begin{equation*}
\begin{split}
\psi^1(X,Y)&=\overline{\psi}_0-\sum_{q\in\mathbb{Z}}\int_{\mathbb{R}}\partial_{Y'}Y'K(X,Y')\dfrac{1}{Y'}\int_0^{Y'}\left(\psi_0(Y-Y_1)-\overline{\psi}_0\right)dY_1\varphi_q(Y')dY'\\
&=\overline{\psi}_0+J.
\end{split}
\end{equation*}
Now, we focus our attention on controlling the term $J$. Here, we have the key estimates 
\begin{align*}\label{15}
&|Y'\partial_Y'K(X,Y')|\leq C\dfrac{X^{1/2}}{X^{1/2}+Y'^2},\quad\forall|X|\geq 1,\quad \forall Y'\in\mathbb{R},\\
&\int_\mathbb{R}Y'\partial_Y'K(X,Y')=-1,\numberthis
\end{align*}
which are easily obtained by following a reasoning similar to one presented earlier in this paragraph.

We conduct the analysis by distinguishing the behavior of $J$ in $|Y'|\leq R$ from the one on $|Y'|\geq R$ for $R\gg 1 $, denoted by $J_1$ and $J_2$ respectively.  We have that $J_1=O(\varepsilon)$, since for $|Y'|\geq R$
\begin{equation*}
\left|\dfrac{1}{Y'}\int_0^{Y'}\left(\psi_0(Y-Y_1)-\overline{\psi}_0\right)dY_1\right|\leq \varepsilon.
\end{equation*}
For $|Y'|\geq R$, we have that 
\begin{equation*}
\left|\dfrac{1}{Y'}\int_0^{Y'}\left(\psi_0(Y-Y_1)-\overline{\psi}_0\right)dY_1\right|\leq 2\|\psi_0\|_{L^1_{\mathrm{uloc}}},
\end{equation*}
hence,
\begin{equation*}
\begin{split}
|J_2|&=\left|\sum_{q\in\mathbb{Z}}\int_{|Y'|\leq R}\partial_{Y'}Y'K(X,Y')\dfrac{1}{Y'}\int_0^{Y'}\left(\psi_0(Y-Y_1)-\overline{\psi}_0\right)dY_1\varphi_q(Y')dY\right|\\
&\leq C\|\psi_0\|_{L^1_{\mathrm{uloc}}}\left|\int_{|Y'|\leq R}\dfrac{X^{1/4}}{X^{1/2}+Y'^{2}}dY'\right|\\
&\leq C_R\|\psi_0\|_{L^1_{\mathrm{uloc}}}|X|^{-1/4}\underset{X\rightarrow\infty}{\longrightarrow} 0.
\end{split}
\end{equation*}
Therefore, we can conclude that \begin{equation*}
\underset{X\rightarrow\infty}{\lim}J(X,Y)=0,\quad\mathrm{and}\quad \underset{X\rightarrow\infty}{\lim}\psi^1(X,Y)(X,Y)=\overline{\psi}_0=
\mathbb{E}[\psi_0]
\end{equation*}
